Prevalence Threshold and the Geometry of Screening Curves

The relationship between a screening tests' positive predictive value, $\rho$, and its target prevalence, $\phi$, is proportional - though not linear in all but a special case. In consequence, there is a point of local extrema of curvature defined only as a function of the sensitivity $a$ and specificity $b$ beyond which the rate of change of a test's $\rho$ drops precipitously relative to $\phi$. Herein, we show the mathematical model exploring this phenomenon and define the $prevalence$ $threshold$ ($\phi_e$) point where this change occurs as: $\phi_e=\frac{\sqrt{a\left(-b+1\right)}+b-1}{(\varepsilon-1)}$ where $\varepsilon$ = $a$+$b$. Using its radical conjugate, we obtain a simplified version of the equation: $\frac{\sqrt{1-b}}{\sqrt{a}+\sqrt{1-b}}$. From the prevalence threshold we deduce a more generalized relationship between prevalence and positive predictive value as a function of $\varepsilon$, which represents a fundamental theorem of screening, herein defined as: $\displaystyle\lim_{\varepsilon \to 2}{\displaystyle \int_{0}^{1}}{\rho(\phi)d\phi} = 1$ Understanding the concepts described in this work can help contextualize the validity of screening tests in real time, and help guide the interpretation of different clinical scenarios in which screening is undertaken.

==> references.tex <==
@article{wilson1968principles,
  title={Principles and practice of screening for disease},
  author={Wilson, James Maxwell Glover and Jungner, Gunnar and World Health Organization and others},
  year={1968},
  publisher={World Health Organization}
}

@article{sackett1975screening,
  title={Screening for early detection of disease: to what purpose?},
  author={Sackett, DAVID L},
  journal={Bulletin of the New York Academy of Medicine},
  volume={51},
  number={1},
  pages={39},
  year={1975},
  publisher={New York Academy of Medicine}
}

@article{andermann2008public,
  title={Public health classics},
  author={Andermann, Anne and Blancquaert, Ingeborg and Beauchampb, Sylvie and D{\'e}ryc, V{\'e}ronique},
  journal={Bulletin of the World Health Organization},
  volume={86},
  number={4},
  year={2008}
}

@article{herman2006makes,
  title={What makes a screening exam" good"?},
  author={Herman, Cheryl},
  journal={AMA Journal of Ethics},
  volume={8},
  number={1},
  pages={34--37},
  year={2006},
  publisher={American Medical Association}
}

@article{brenner1997variation,
  title={Variation of sensitivity, specificity, likelihood ratios and predictive values with disease prevalence},
  author={Brenner, Hermann and Gefeller, OLAF},
  journal={Statistics in medicine},
  volume={16},
  number={9},
  pages={981--991},
  year={1997},
  publisher={Wiley Online Library}
}

@article{moons1997limitations,
  title={Limitations of sensitivity, specificity, likelihood ratio, and Bayes' theorem in assessing diagnostic probabilities: a clinical example},
  author={Moons, Karel GM and van Es, Gerrit-Anne and Deckers, Jaap W and Habbema, J Dik F and Grobbee, Diederick E},
  journal={Epidemiology},
  pages={12--17},
  year={1997},
  publisher={JSTOR}
}

@article{cheng2020diagnostic,
  title={Diagnostic testing for severe acute respiratory syndrome--related coronavirus-2: A narrative review},
  author={Cheng, Matthew P and Papenburg, Jesse and Desjardins, Micha{\"e}l and Kanjilal, Sanjat and Quach, Caroline and Libman, Michael and Dittrich, Sabine and Yansouni, Cedric P},
  journal={Annals of internal medicine},
  year={2020},
  publisher={American College of Physicians}
}

@article{smith2000first,
  title={The first positive: computing positive predictive value at the extremes},
  author={Smith, James E and Winkler, Robert L and Fryback, Dennis G},
  journal={Annals of internal medicine},
  volume={132},
  number={10},
  pages={804--809},
  year={2000},
  publisher={American College of Physicians}
}

@article{cheng2020diagnostic,
  title={Diagnostic testing for severe acute respiratory syndrome--related coronavirus-2: A narrative review},
  author={Cheng, Matthew P and Papenburg, Jesse and Desjardins, Micha{\"e}l and Kanjilal, Sanjat and Quach, Caroline and Libman, Michael and Dittrich, Sabine and Yansouni, Cedric P},
  journal={Annals of internal medicine},
  year={2020},
  publisher={American College of Physicians}
}
